How Tokenization Limits Phonological Knowledge Representation in Language Models and How to Improve Them

Tokenization is the first step in every language model (LM), yet it never takes the sounds of words into account. We investigate how tokenization influences text-only LMs' ability to represent phonological knowledge. Through a series of probing experiments, we show that subword-based tokenization systematically weakens the encoding of both local (e.g., rhyme) and global (e.g., syllabification) phonological features. To quantify this effect, we introduce the syllabification-tokenization alignment distance (STAD), a metric that measures the misalignment between a model's tokenization and the natural syllable boundaries of words, and find that higher misalignment correlates with poorer phonological representations, providing a simple diagnostic for phonology-aware tokenization. To address these limitations, we propose a lightweight IPA-based fine-tuning method that infuses phonological awareness into LMs, leading to consistent improvements across three phonology-related tasks while largely preserving math and general reasoning ability, with 1.1\% and 0.9\% drops on GSM8K and MMLU, respectively.

==> table/prbing_rhyming_awareness.tex <==
\definecolor{mygray}{gray}{0.85}  % Light gray
\begin{table}[!h]
    \setlength{\tabcolsep}{3pt}
    \footnotesize
    \centering
    % \alternaterowcolors
    \begin{tabular}{cc|cccccc}
        \toprule
        \textbf{Model} & \textbf{Format} & \multicolumn{6}{c}{\textbf{Depth} (Accuracy $\uparrow$)}                                                                                                                                            \\
        \cmidrule(lr){3-8}
        \textbf{Size}  &                 & 0\%                                                      & 20\%                       & 40\%                         & 60\%                         & 80\%                       & 100\%            \\
        \midrule
        \multicolumn{8}{c}{Subword Tokenization}                                                                                                                                                                                               \\
        \midrule
        \rowcolor{mygray}
        \multicolumn{8}{l}{\textbf{BERT}}                                                                                                                                                                                                      \\
        110M           & Orig            & 56.0                                                     & 67.6                       & 68.3                         & 70.9                         & \underline{71.0}           & 70.5             \\
                       & Slash           & \threestar{68.6}                                         & \twostar{74.5}             & \twostar{73.4}               & \twostar{77.5}               & \underline{\twostar{79.5}} & \twostar{78.1}   \\
        \rowcolor{mygray}
        \multicolumn{8}{l}{\textbf{GPT2}}                                                                                                                                                                                                      \\
        1.2B           & Orig            & 63.4                                                     & 64.7                       & 66.1                         & \underline{66.2}             & 66.0                       & 61.6             \\
                       & Slash           & \threestar{71.7}                                         & \threestar{76.9}           & \threestar{77.2}             & \underline{\threestar{79.1}} & \threestar{78.5}           & \threestar{77.5} \\
        \midrule
        \rowcolor{mygray}
        \multicolumn{8}{l}{\textbf{GPT-neo-2.7b}}                                                                                                                                                                                              \\
        2.7B           & Orig            & 68.2                                                     & 68.6                       & \underline{72.4}             & 69.6                         & 69.7                       & 67.0             \\
                       & Slash           & 73.2                                                     & \threestar{82.5}           & \underline{\threestar{83.9}} & \threestar{82.5}             & \threestar{81.6}           & \threestar{82.4} \\
        \rowcolor{mygray}
        \multicolumn{8}{l}{\textbf{Llama3-8b-Instruct}}                                                                                                                                                                                        \\
        8B             & Orig            & 71.4                                                     & \underline{80.7}           & 76.6                         & 76.8                         & 70.5                       & 78.4             \\
                       & Slash           & 56.3                                                     & \underline{\onestar{85.4}} & \twostar{81.9}               & \textbf{77.9}                & \textbf{71.9}              & 76.1             \\
        \midrule
        \rowcolor{mygray}
        \multicolumn{8}{l}{\textbf{Llama3.1-8b-Instruct}}                                                                                                                                                                                      \\
        8B             & Orig            & 72.5                                                     & \underline{79.8}           & 79.0                         & 77.9                         & 77.3                       & 74.9             \\
                       & Slash           & 56.3                                                     & \underline{\twostar{85.1}} & \twostar{84.0}               & \textbf{80.0}                & \textbf{78.9}              & \twostar{79.5}   \\
        \midrule
        \rowcolor{mygray}
        \multicolumn{8}{l}{\textbf{Mistral-7b-Instruct-v3}}                                                                                                                                                                                    \\
        7B             & Orig            & 64.5                                                     & 80.6                       & \underline{80.8}             & 78.8                         & 77.4                       & 74.7             \\
                       & Slash           & 55.8                                                     & \textbf{81.1}              & \underline{\onestar{82.7}}   & \textbf{79.5}                & \onestar{79.0}             & \twostar{77.6}   \\
        \midrule
        \multicolumn{8}{c}{Character Tokenization}                                                                                                                                                                                             \\
        \midrule
        \rowcolor{mygray}
        \multicolumn{8}{l}{\textbf{ByT5-base}}                                                                                                                                                                                                 \\
        580M           & Orig            & 45.5                                                     & 79.6                       & \underline{81.0}             & 79.9                         & 80.3                       & 66.3             \\
                       & Slash           & -                                                        & -                          & -                            & -                            & -                          & -                \\
        \midrule
        \rowcolor{mygray}
        \multicolumn{8}{l}{\textbf{ByT5-small}}                                                                                                                                                                                                \\
        300M           & Orig            & 45.5                                                     & 75.5                       & \underline{80.1}             & 77.6                         & 72.7                       & 71.8             \\
                       & Slash           & -                                                        & -                          & -                            & -                            & -                          & -                \\
        \midrule
        \multicolumn{8}{c}{Control Experiment}                                                                                                                                                                                                 \\
        \midrule
        \rowcolor{mygray}
        \multicolumn{8}{l}{\textbf{Random Embeddings}}                                                                                                                                                                                         \\
        -              & -               & 48.8                                                     & 48.7                       & 51.7                         & 49.3                         & 50.2                       & 50.8             \\
        \bottomrule
    \end{tabular}
    \caption{Accuracy of logistic regression trained on language models of varying depths, comparing performance with words containing slash separators (Slash) vs. original words (Orig).
        The reported values are the average accuracy over 10 runs.
        \textbf{Bold} indicates that Slash outperforms Orig, while \underline{underlined} values denote the highest accuracy in each row. A t-test is conducted to assess the hypothesis that Slash achieves higher accuracy than Orig, with significance levels indicated as follows: $p < 0.05$ (*), $p < 0.01$ (**), and $p < 0.001$ (***). We also include the results of 32-layers of randomized embeddings, and the results is almost random guess, meaning that our linear prober is not overfitting to the task.}
    \label{table:table_rhyme}
\end{table}


==> table/probing_rhyming.tex <==
\begin{table*}[!h]
\setlength{\tabcolsep}{5pt}
    \footnotesize
    \centering
\begin{tabular}{l|c|cc|cc|cc|cc|cc|cc}
\toprule
\textbf{Model} & \textbf{Size} & \multicolumn{2}{c}{\textbf{0\% depth}} & \multicolumn{2}{c}{\textbf{20\% depth}} & \multicolumn{2}{c}{\textbf{40\% depth}} & \multicolumn{2}{c}{\textbf{60\% depth}} & \multicolumn{2}{c}{\textbf{80\% depth}} & \multicolumn{2}{c}{\textbf{100\% depth}} \\
\cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} \cmidrule(r){11-12} \cmidrule(r){13-14}
& & Orig & Slash & Orig & Slash & Orig & Slash & Orig & Slash & Orig & Slash & Orig & Slash \\
\midrule
\multicolumn{14}{c}{Subword Tokenization} \\
\midrule
% \midrule
\textbf{gpt2} & 1.2B & 63.4 & 71.7 & 64.7 & 76.9 & 66.1 & 77.2 & 66.23 & 79.13 & 66.03 & 78.5 & 61.63 & 77.5 \\
\textbf{llama3} & 7B & 58.5 & 55.3 & 76.6 & 78.0 & 74.8 & 78.7 & 72.8 & 73.8 & 70.5 & 71.9 & 69.9 & 69.9 \\
\textbf{llama3.1} & 8B & 64.7 & 56.3 & 76.4 & 80.8 & 73.9 & 76.7 & 73.9 & 72.7 & 73.8 & 69.2 & 69.5 & 69.3 \\
\textbf{mT5} & 200M & 49.1 & 49.1 & 65.2 & 70.6 & 66.8 & 73.4 & 66.3 & 72.9 & 65.4 & 72.1 & 64.6 & 73.4 \\
\midrule
\multicolumn{14}{c}{Character Tokenization} \\
\midrule
\textbf{ByT5-base} & 400M & 49.1 & NA & 72.9 & NA & 74.9 & NA & 74.4 & NA & 68.3 & NA & 66.3 & NA \\
\textbf{ByT5-small} & 49.1 & 49.1 & NA & 68.9 & NA & 73.1 & NA & 72.7 & NA & 69.2 & NA & 69.5 & NA \\
\bottomrule
\end{tabular}
\caption{Accuracy for Different Depth (orig/slash) with Added Columns and No Vertical Lines}
\end{table*}
